Numerical scheme for treatment of Uehling-Uhlenbeck equation for two-particle interactions in relativistic plasma

We present a new efficient method to compute Uehling-Uhlenbeck collision integral for all two-particle interactions in relativistic plasma with drastic improvement in computation time with respect to existing methods. Plasma is assumed isotropic in momentum space. The set of reactions consists of: Moeller and Bhabha scattering, Compton scattering, two-photon pair annihilation, and two-photon pair production, which are described by QED matrix elements. In our method exact energy and particle number conservation laws are satisfied. Reaction rates are compared, where possible, with the corresponding analytical expressions and convergence of numerical rates is demonstrated.

==> chap1.tex <==
\section{Abstract}\label{ch1}

We present a new efficient method to compute Boltzmann collision integral for all two-particle interactions in relativistic plasma. Plasma is assumed to be homogeneous in coordinate space and isotropic in momentum space. The set of reactions consists of: Moeller and Bhabha scattering, Compton scattering, two-photon pair annihilation, and two-photon pair production, which are described by QED matrix elements. In our method exact energy and particle number conservation laws are fulfilled. Drastic improvement in computation time with respect to existing methods is achieved. Reaction rates are compared, where possible, with the corresponding analytical expressions and convergence of numerical rates is demonstrated.
